Joint Passage Ranking for Diverse Multi-Answer Retrieval

We study multi-answer retrieval, an under-explored problem that requires retrieving passages to cover multiple distinct answers for a given question. This task requires joint modeling of retrieved passages, as models should not repeatedly retrieve passages containing the same answer at the cost of missing a different valid answer. In this paper, we introduce JPR, the first joint passage retrieval model for multi-answer retrieval. JPR makes use of an autoregressive reranker that selects a sequence of passages, each conditioned on previously selected passages. JPR is trained to select passages that cover new answers at each timestep and uses a tree-decoding algorithm to enable flexibility in the degree of diversity. Compared to prior approaches, JPR achieves significantly better answer coverage on three multi-answer datasets. When combined with downstream question answering, the improved retrieval enables larger answer generation models since they need to consider fewer passages, establishing a new state-of-the-art.

==> sections/12-examples.tex <==
who was british pm and viceroy during quit india movement
Answers: [['winston churchill'], ['lord linlithgow', 'linlithgow', 'victor hope 2nd marquess of linlithgow', 'victor alexander john hope 2nd marquess of linlithgow']]
Answers: [['linlithgow', 'victor alexander john hope', 'victor hope 2nd marquess of linlithgow'], ['sir winston leonard spencerchurchill', 'winston churchill']]
1.0 0.5


In [2]: prediction1["blocks"][0]
Out[2]:
{'title': 'Quit India Movement',
 'text': 'Quit India Movement\n\nThe Quit India Movement, or the India August Movement, was a movement launched at the Bombay session of the All-India Congress Committee by Mahatma Gandhi on 8 \nAugust 1942, during World War II, demanding an end to British Rule of India. The Cripps Mission had failed, and on August 8, 1942, Gandhi made a call to "Do or Die" in his Quit India speech delivered in Bombay at the Gowalia Tank Maidan. The All-India Congress Committee launched a mass protest demanding what Gandhi called "An Orderly British Withdrawal" from India. Even though it was wartime, the British were prepared to act. Almost the entire leadership of the Indian National Congress was imprisoned without trial within hours of Gandhi\'s speech. Most spent the rest of the war in prison and out ofcontact with the masses. The British had the support of the Viceroy\'s Council (which had a majority of Indians), of the All India Muslim League, the princely states, the IndianImperial Police, the British Indian Army and the Indian Civil Service. Many Indian businessmen profiting from heavy wartime spending did not support the Quit India Movement. Many students paid more attention to Subhas Chandra Bose, who was in exile and supporting the Axis Powers. The only outside support came from the Americans, as President Franklin D.Roosevelt pressured Prime Minister Winston Churchill to give in to some of the Indian demands.',
 'block_id': 8021734,
 'score': 1.0}
 
 
 ': 'Quit India Movement',
 'text': 'Responding to this declaration, the Viceroy issued a statement on 17 October wherein he claimed that Britain is waging a war driven with the intention of strengtheningpeace in the world. He also stated that after the war, the government would initiate modifications in the Act of 1935, in accordance to the desires of the Indians. Gandhi\'s reaction to this statement was; "the old policy of divide and rule is to continue. The Congress has asked for bread and it has got stone." According to the instructions issued by High Command, the Congress ministers were directed to resign immediately. Congress ministers from eight provinces resigned following the instructions. The resignation of the ministers was an occasion of great joy and rejoicing for leader of the Muslim League, Mohammad Ali Jinnah. He called the day of 22 December 1939 \'The Day of Deliverance\'. Gandhi urged Jinnah against the celebration of this day, however, it was futile. At the Muslim League Lahore Session held in March 1940, Jinnah declared in his presidential address that theMuslims of the country wanted a separate homeland, Pakistan. In the meanwhile, crucial political events took place in England. Chamberlain was succeeded by Churchill as prime minister and the Conservatives, who assumed power in England, did not have a sympathetic stance towards the claims made by the Congress.',
 'block_id': 8021738,
 'score': 0.9090909090909091}

...

last block:

In [5]: prediction1["blocks"][-1]
Out[5]:
{'title': 'Cripps Mission',
 'text': 'Jinnah and the Muslims, to whom Cripps had offered the right to opt out of a future Union, supported the war effort and gained in status in British eyes. He was "surprised" to see that the right to opt out of a future Union was included. The Government of India Act 1935 - building on the Round Table Conferences, Simon Commission and the previous Government of India Act of 1919 - required the establishment of an All-India Federation, which would allow Indians to take a larger share of governance at the highest level. However deep difference between the princely states and the Congress, as well as between the Muslim League and Congress, had delayed progress. Instead, only the provincial portionof the Act was carried out. Following Britain\'s declaration of war on Germany in September 1939, the Viceroy, Lord Linlithgow, responded by declaring India a belligerent state on the side of Britain without consulting Indian political leaders or the elected provincial representatives, sharply underlying the failure of progress to self-rule. This causedconsiderable resentment in the Congress Party, producing demands for an immediate transfer of power. The resulting standoff led to the en masse resignation of Congress Provincial Governments, giving rise to the prospect of public revolt and political disorder in India.',
 'block_id': 1048669,
 'score': 0.7142857142857143}




baseline:

In [6]: prediction2["blocks"][0]
Out[6]:
{'title': 'Quit India Movement',
 'text': 'Quit India Movement\n\nThe Quit India Movement, or the India August Movement, was a movement launched at the Bombay session of the All-India Congress Committee by Mahatma Gandhi on 8 \nAugust 1942, during World War II, demanding an end to British Rule of India. The Cripps Mission had failed, and on August 8, 1942, Gandhi made a call to "Do or Die" in his Quit India speech delivered in Bombay at the Gowalia Tank Maidan. The All-India Congress Committee launched a mass protest demanding what Gandhi called "An Orderly British Withdrawal" from India. Even though it was wartime, the British were prepared to act. Almost the entire leadership of the Indian National Congress was imprisoned without trial within hours of Gandhi\'s speech. Most spent the rest of the war in prison and out ofcontact with the masses. The British had the support of the Viceroy\'s Council (which had a majority of Indians), of the All India Muslim League, the princely states, the IndianImperial Police, the British Indian Army and the Indian Civil Service. Many Indian businessmen profiting from heavy wartime spending did not support the Quit India Movement. Many students paid more attention to Subhas Chandra Bose, who was in exile and supporting the Axis Powers. The only outside support came from the Americans, as President Franklin D.Roosevelt pressured Prime Minister Winston Churchill to give in to some of the Indian demands.',
 'block_id': 8021734,
 'score': -1.0728836059570312e-06}

....


{'title': 'British Raj',
 'text': "The British government sent the Cripps' mission in 1942 to secure Indian nationalists' co-operation in the war effort in exchange for a promise of independence as soonas the war ended. Top officials in Britain, most notably Prime Minister Winston Churchill, did not support the Cripps Mission and negotiations with the Congress soon broke down.Congress launched the Quit India Movement in July 1942 demanding the immediate withdrawal of the British from India or face nationwide civil disobedience. On 8 August the Raj arrested all national, provincial and local Congress leaders, holding tens of thousands of them until 1945. The country erupted in violent demonstrations led by students and later by peasant political groups, especially in Eastern United Provinces, Bihar, and western Bengal. The large wartime British Army presence crushed the movement in a little more thansix weeks; nonetheless, a portion of the movement formed for a time an underground provisional government on the border with Nepal. In other parts of India, the movement was less spontaneous and the protest less intensive, however it lasted sporadically into the summer of 1943. It did not slow down the British war effort or recruiting for the army. Earlier, Subhas Chandra Bose, who had been a leader of the younger, radical, wing of the Indian National Congress in the late 1920s and 1930s, had risen to become Congress President from 1938 to 1939.",
 'block_id': 3788696,
 'score': -2.0116567611694336e-05}




------------------



when does the new family guy season come out
Answers: [['october 1 2017'], ['september 25 2016'], ['september 27 2015']]
1.0 0.3333333333333333
Ours
('Family Guy (season 16)', ['october 1 2017'])
('Family Guy (season 14)', ['september 27 2015'])
('Family Guy (season 13)', [])
('Family Guy (season 17)', [])
('Family Guy (season 15)', ['september 25 2016'])
Base
('Family Guy (season 16)', ['october 1 2017'])
('Family Guy (season 17)', [])
('Family Guy', [])
('Emmy-Winning Episode', ['october 1 2017'])
('A House Full of Peters', [])
Python 3.7.9 (default, Aug 31 2020, 12:42:55)

----------------------------


who is the current environmental minister of india
Answers: [['vardhan', 'harsh vardhan', 'dr harsh vardhan'], ['anil madhav dave', 'dave'], ['prakash keshav javadekar', 'prakash javadekar', 'javadekar']]
Answers: [['dr harsh vardhan'], ['anil madhav dave'], ['prakash keshav javadekar', 'prakash javadekar']]
1.0 0.6666666666666666
Ours
('Ministry of Environment, Forest and Climate Change', ['vardhan', 'harsh vardhan', 'dr harsh vardhan', 'dr harsh vardhan'])
('INS Kadamba', ['prakash javadekar', 'javadekar', 'prakash javadekar'])
('Asbestos and the law', ['anil madhav dave', 'dave', 'anil madhav dave'])
('Ricky Kej', ['vardhan', 'harsh vardhan', 'dr harsh vardhan', 'dr harsh vardhan'])
('Narcondam Island', ['prakash javadekar', 'javadekar', 'prakash javadekar'])
Base
('Ministry of Environment, Forest and Climate Change', ['vardhan', 'harsh vardhan', 'dr harsh vardhan', 'dr harsh vardhan'])
('Ricky Kej', ['vardhan', 'harsh vardhan', 'dr harsh vardhan', 'dr harsh vardhan'])
('Harsh Vardhan (Delhi politician)', ['vardhan', 'harsh vardhan', 'dr harsh vardhan', 'dr harsh vardhan'])
('Prakash Javadekar', ['prakash javadekar', 'javadekar', 'prakash javadekar'])
('INS Kadamba', ['prakash javadekar', 'javadekar', 'prakash javadekar'])
Python 3.7.9 (default, Aug 31 2020, 12:42:55)

-------------------------------------------------


what language tunisia
Answers: [['french'], ['arabic language']]
1.0 0.5
Ours
('National language', ['french'])
('Turks in Tunisia', [])
('Languages of Tunisia', ['french', 'arabic language'])
('Tunisian Arabic', ['french', 'arabic language'])
('Demographics of Africa', ['arabic language'])
Base
('National language', ['french'])
('Culture of Tunisia', ['french'])
('Tunisian Arabic', [])
('History of French-era Tunisia', ['french'])
('Geographical distribution of French speakers', ['french'])
Python 3.7.9 (default, Aug 31 2020, 12:42:55)



Out[1]:
{'title': 'National language',
 'text': 'The Romansh speakers are concentrated in the Canton of Grisons in the south-east. During Japanese rule (1895 to 1945), the promoted the Japanese language. After their defeat in the Chinese Civil War in 1949, the Kuomintang regime of the Republic of China retreated to the island of Taiwan, where they introduced Standard Chinese, which was spoken by few of the island population at the time, as the new "national language". In 2017, the Indigenous languages and Taiwanese Hakka were recognized as national languages. The official language of the Tunisian state is Arabic. However, that language is not the mothertongue of the population or used to communicate between Tunisian people, instead Tunisian Arabic plays these roles and is the national language of Tunisia. Also, even without anofficial status, French is also used extensively in its written and spoken form in the administration, education and business environment and known by 63.6% of the population. Also Berber minorities in the south-west and on Djerba Island use the Tunisian Chelha language to communicate between themselves. Turkish is the national language of Turkey per the Turkish constitution. The English language (British English) is the "de facto" officiallanguage of the United Kingdom and is the sole language of an estimated 95% of the British population.',
 'block_id': 7643572,
 'score': 1.0}



{'title': 'Turks in Tunisia',
 'text': 'Turks in Tunisia\n\nThe Turks in Tunisia, also known as Turco-Tunisians and Tunisian Turks, (; ; ) are the ethnic Turks who constitute a group in Tunisia. In 1534, with about 10,000 Turkish soldiers, the Ottoman Empire took control and settled in the region when Tunisia\'s inhabitants called for help due to fears that the Spanish would invade the country. Thus, during the Ottoman rule, the Turks colonized and dominated the political life of the region for centuries; as a result, the ethnic mix of Tunisia changed with the migration of Turks from Anatolia and the evolvement of the "Kouloughlis" who are people of mixed Turkish and central Tunisian blood. In northern Cap Bon, the town of Hammam Ghezèze ( "Oghuz\'s bath") is populated with descendants of Oghuz Turks ("Ghezèze" and "Aghzaz" being Arabic for "Oghuz"). Families of Turkish origin live mainly near the coastal cities, such as Tunis, Mahdia, Hammamet and the islands (such as Djerba), although there are also many living within central Tunisia as well. In 2012 the Tunisian government introduced the Turkish language in all Tunisian secondary schools.',
 'block_id': 3539939,
 'score': 0.9090909090909091}



ut[3]:
{'title': 'Languages of Tunisia',
 'text': "They are also spoken in some hamlets on the island of Djerba, mainly Guellala,Iquallalen, Ajim, Sedouikech, Azdyuch and Ouirsighen. During the French protectorate of Tunisia, French was introduced in public institutions, most notably the education system,which became a strong vehicle for dissemination of the language. From independence, the country gradually became arabized even though the public administration and education remained bilingual. Meanwhile, knowledge of French and other European languages (such as English and Italian) is enhanced by Tunisia's proximity to Europe and by media and tourism. The 1990s marked a turning point for the Arabization process. Science classes up to the end of middle school were Arabized in order to facilitate access to higher education and promote the Arabic language in society. Since October 1999, private establishments have been obliged to give Arabic characters twice the size of Latin characters. This rule is notalways followed, however. At the same time, the public administration is required to communicate in Arabic only. In this context, the use of French seems to be in decline despite the increased number of graduates in the educational system, which leads to the fact that a good knowledge of French remains an important social marker. This is because French is widely used in the business community, intellectual domains and the spheres of naturalscience and medicine.",
 'block_id': 3102373,
 'score': 0.8333333333333334}

 'score': 0.8333333333333334}

In [4]: prediction1["blocks"][3]
Out[4]:
{'title': 'Tunisian Arabic',
 'text': "However, code-switching between Tunisian Arabic and modern standard Arabic is mainly done by more educated and upper-class people and has not negatively affected the use of more recent French and English loanwords in Tunisian. Moreover, Tunisian Arabic is closely related to Maltese, which is a separate language that descended from Tunisian andSiculo-Arabic. Tunisian Arabic is one of the Arabic languages within the Semitic branch of the Afroasiatic language family. It is a variety of Maghrebi Arabic like Moroccan and Algerian Arabic, which are mostly unintelligible to Modern Standard or Mashriqi Arabic speakers. It has a considerable number of pre-hilalian dialects but is usually considered in its koiné form to be a mostly Hilalian variety of Maghrebi Arabic because it was affected by the immigration of Banu Hilal in the 11th century, as were the other Maghrebi varieties. As a part of the Arabic dialect continuum, it is reported that Tunisian Arabic is partly mutually intelligible with Algerian Arabic, Libyan Arabic and Maltese. However, it is slightly intelligible or even not intelligible with Moroccan, Egyptian, Levantine, Mesopotamian, or Gulf Arabic. During classical antiquity, Tunisia's population spoke Berber languages related to the Numidian language.",
 'block_id': 9513076,
 'score': 0.7692307692307693}



In [5]: prediction1["blocks"][4]
Out[5]:
{'title': 'Demographics of Africa',
 'text': "In the central Sahara, Mandinka or Mande groups are most significant. Chadic-speaking groups, including the Hausa, are found in the more northerly parts of the region nearest to the Sahara and Nilo-Saharan communities such as the Kanuri, Zarma and Songhai are present in eastern parts of West Africa bordering Central Africa. The peoples of North Africa comprise three main groups: Berbers in the northwest, Egyptians and Libyans in northeast, and Nilo-Saharan-speaking peoples in the east. The Muslim settlers who arrived in the 7th century introduced the Arabic language and Islam to the region, initiating a process of linguistic Arabization of the region's inhabitants. The Semitic Phoenicians (who founded Carthage) and Hyksos, the Indo-Iranian Alans, the Indo-European Greeks, Romans and Vandals settled in North Africa as well. Berber-speaking populations still make significant communities within Morocco and Algeria and are still also present in smaller numbers in Tunisia and Libya. The Berber-speaking Tuareg and other often-nomadic peoples are the principal inhabitants of the Saharan interior of North Africa. In Mauritania, there isa small Berber community and Niger–Congo-speaking peoples in the South, though in both regions Arabic and Arab culture predominates.",
 'block_id': 5742017,
 'score': 0.7142857142857143}




-----------------------------


 prediction2["blocks"][0]
Out[6]:
{'title': 'National language',
 'text': 'The Romansh speakers are concentrated in the Canton of Grisons in the south-east. During Japanese rule (1895 to 1945), the promoted the Japanese language. After their defeat in the Chinese Civil War in 1949, the Kuomintang regime of the Republic of China retreated to the island of Taiwan, where they introduced Standard Chinese, which was spoken by few of the island population at the time, as the new "national language". In 2017, the Indigenous languages and Taiwanese Hakka were recognized as national languages. The official language of the Tunisian state is Arabic. However, that language is not the mothertongue of the population or used to communicate between Tunisian people, instead Tunisian Arabic plays these roles and is the national language of Tunisia. Also, even without anofficial status, French is also used extensively in its written and spoken form in the administration, education and business environment and known by 63.6% of the population. Also Berber minorities in the south-west and on Djerba Island use the Tunisian Chelha language to communicate between themselves. Turkish is the national language of Turkey per the Turkish constitution. The English language (British English) is the "de facto" officiallanguage of the United Kingdom and is the sole language of an estimated 95% of the British population.',
 'block_id': 7643572,
 'score': -1.1868774890899658e-05}


 prediction2["blocks"][1]
Out[7]:
{'title': 'Culture of Tunisia',
 'text': 'The country is characterized by its tolerance and openness to other cultures. For instance, the teaching of Islam is compulsory in public schools but the program of religious studies at the secondary level also includes the history of Judaism and Christianity. The Tunisians also retain some native beliefs of Berber origin such as the evil eye.A number of practices, such as shutters painted blue are also used to repel evil spirits. Tunisia is homogeneous in terms of language, since nearly all of the population mastersFrench and Arabic (the state Official language) and speaks Tunisian Arabic which is the mother-tongue of almost all Tunisians. Tunisian Arabic is actually a dialect - or more accurately a set of dialects, for which there is no official body of standards. It is established on a berber and punic substratum, influenced by the languages of the people that lived or administered the region, during the course of history, including: Arabic, Turkish, Italian, Spanish and French. Tunisian Arabic is not understood by most Arab speaking countries as it does derive from a mixture of a few languages. Tunisian is spoken mostly inthe context of a daily dialogue between Tunisians and within the family.',
 'block_id': 2503805,
 'score': -1.2271106243133545e-05}

In [8]:



{'title': 'Tunisian Arabic',
 'text': 'The Hilalian set includes the Sulaym dialects in the south and the Eastern Hilal dialects in central Tunisia. The latter were also spoken in the Constantinois (easternAlgeria). Nowadays and due to dialect leveling, the main dialect varieties of Tunisian Arabic are Northwestern Tunisian (also spoken in Northeastern Algeria), southwestern Tunisian, Tunis dialect, Sahil dialect, Sfax dialect and southeastern Tunisian. All of these varieties are Hilalian excepting the Sfax one. Tunis, Sahil and Sfax dialects (considered sedentary dialects) use the voiceless uvular stop in words such as قال "he said" while southeastern, northwestern and southwestern varieties (considered nomadic dialects) substitute it by the voiced velar stop as in . Moreover, only Tunis, Sfax and Sahil dialects useTunisian phonology. Indeed, northwestern and southwestern Tunisians speak Tunisian with Algerian Arabic phonology, which tends to simplify short vowels as short schwas while southeastern Tunisian speak Tunisian with the Libyan Arabic phonology. Additionally, Tunis, Sfax and the urban Sahil dialects are known for not marking the second person gender. Hence, the otherwise feminine إنتِي is used to address both men and women, and no feminine marking is used in verbs ("inti mšīt").',
 'block_id': 9513087,


'History of French-era Tunisia',
 'text': 'Similar issues arose later in Tunisia, including the views of the national movement. In Tunisia the French in 1883 set up a "Direction de l\'Enseignement Public" (Directorate of Public Education) to promote schools for teaching children of French officialsand colons, and to further the spreading use of the French language. Its goals widened to include education in general. This Directorate eventually administered, or directed, all the different educational institutions and systems in Tunisia, which it sought to modernize, coordinate, grow and expand. Soon established in Tunis were the new mixed Collège Alaoui, and for women the new École Rue du Pacha and École Louise René Millet. Several separate educational systems eventually resulted under the Protectorate. Serving French "colons" and Tunisians was a primary and secondary system closely coordinated with Metropolitan France, using the French language. From here students might attend a university in France. The government also directed a modern secular system of schools using mixed French and Arabic. The "kuttab" primary schools remained, keeping their religious instruction, yet enhanced by arithmetic, history, French, and hygiene; taught primarily in Arabic, the "kuttab" received government support. Thus Zitouna Mosque students might come from either the mixed secular or the "kuttab" religious schools.',
 'block_id': 4773765,


: 'Geographical distribution of French speakers',
 'text': 'Teachers are not always sufficiently trained for this usage, however. Nearly three-quarters of the population of Tunis, Sousse and Sfax consider French as essential intheir professional or personal lives. However, only half of the population feels Francophone, and only a third feels solidarity with other Francophone countries. 70.8% of the population over 15 in the aforementioned Tunisians cities can read and write French. Arabicincreasingly dominates the Tunisian media landscape, especially on television: the audience share of local French-language channels reached 25% in the early 1990s, but hardly reached 3% by the 2010s. On social media, French was used on Facebook by 91% of Tunisians in 2014. Local French-language media include La Presse de Tunisie, L\'Economiste Maghrébin, Tunivisions, Le Temps. According to the High Council of the International Organization of the Francophonie, in 2010, 96.2 million French speakers were living in various countries in Africa. French has been imported to most of these countries through colonization, and it is not a mother tongue to most residents. African standards of French differ from European ones. Some linguists discuss a "second French language" or even an "African French language".',
 'block_id': 2911630,
 'score': -1.2673437595367432e-05}


what is the name of the speaker of the house of representatives now 2011
Answers: [['nancy pelosi'], ['john boehner']]
1.0 0.5
Ours
('Paul Ryan', ['john boehner'])
('John Boehner', ['john boehner'])
('2009 Speaker of the British House of Commons election', [])
('Ripon Society', ['john boehner'])
('Presidency of Barack Obama', ['nancy pelosi', 'john boehner'])
Base
('Paul Ryan', ['john boehner'])
('Freedom Caucus', ['john boehner'])
('History of the United States Republican Party', ['john boehner'])
('United States debt-ceiling crisis of 2013', ['john boehner'])
('October 2015 Speaker of the United States House of Representatives election', ['john boehner'])
Python 3.7.9 (default, Aug 31 2020, 12:42:55)
Type 'copyright', 'credits' or 'license' for more information
IPython 7.18.1 -- An enhanced Interactive Python. Type '?' for help.



